Deep learning based workflow for accelerated industrial X-ray Computed Tomography

X-ray computed tomography (XCT) is an important tool for high-resolution non-destructive characterization of additively-manufactured metal components. XCT reconstructions of metal components may have beam hardening artifacts such as cupping and streaking which makes reliable detection of flaws and defects challenging. Furthermore, traditional workflows based on using analytic reconstruction algorithms require a large number of projections for accurate characterization - leading to longer measurement times and hindering the adoption of XCT for in-line inspections. In this paper, we introduce a new workflow based on the use of two neural networks to obtain high-quality accelerated reconstructions from sparse-view XCT scans of single material metal parts. The first network, implemented using fully-connected layers, helps reduce the impact of BH in the projection data without the need of any calibration or knowledge of the component material. The second network, a convolutional neural network, maps a low-quality analytic 3D reconstruction to a high-quality reconstruction. Using experimental data, we demonstrate that our method robustly generalizes across several alloys, and for a range of sparsity levels without any need for retraining the networks thereby enabling accurate and fast industrial XCT inspections.

==> extra.tex <==
\vspace{-0.25cm}
\section{X-ray CT Scan Challenges}

In this section, we briefly describe some of the common challenges with X-ray CT scanning and reconstruction and describe our solution to mitigate these challenges.

\vspace{-0.25cm}
\subsection{Beam hardening}

With dense metals there is an inherent beam hardening of polychromatic X-rays. 
Lower energy X-rays are absorbed more than higher energy ones, causing the normalized projection value ($p$) to lose the linear relation with the thickness ($d$) of the metal component, rendering the $p\ \text{vs}\ d$ curve non-linear.
This results in cupping and streaking artifacts in the image that could hinder the detection of defects. 
Several approaches, hardware or algorithm-based, are currently employed to mitigate the beam hardening problem. 
Pre-hardening of the x-ray beam involves the use of a metal plate between the component and the x-ray source the lowest-kV x-rays \cite{hsieh2003computed}. 
It could lead to a loss of contrast in the reconstruction image, and also a decrease in signal to noise ratio (SNR). 
Another method comprises of the use of x-ray CT with energy-discriminating detectors, \cite{willemink2018photon, rahman2020direct} which still requires knowledge of the material and its behavior in the x-ray energy bins used. 
One of the popular and inexpensive software-based BH correction is the linearization method \cite{herman1979correction}. 
Using a phantom of the same material and calibration, one can pre-estimate the coefficients of a heuristic polynomial that ``linearizes'' the $p\ \text{vs}\ d$ curve.
Alternatively, \cite{jin2015model} models the non-linearities of the image formation process to reduce BH but is computationally expensive. 
All of the above methods require knowledge of the material of interest or are computationally expensive.

\vspace{-0.25cm}
\subsection{Artifacts from sparse scan}

A reliable X-ray CT scan of thick/dense metal AM components could take hours which makes the defect characterization slow.
This can be solved by reducing the number of projection views (sparse-scan
X-ray CT). 
But this presents its own problems such as using an analytical reconstruction creates sparse-view artifacts in the image that look like streaks. 
Traditionally it is solved by interpolating the sinogram \cite{brooks1978new, kostler2006adaptive, lee2018deep} before the reconstruction step. Another approach is correction of sparse-view artifacts post-reconstruction in the image domain \cite{grant2010iterative, zhang2018sparse}. 
Iterative methods such as MBIR \cite{thibault2007three,yu2010fast} can handle sparse-view artifacts better than analytical methods.
MBIR typically has a pleasing image texture but because of the iterative nature it takes a long time and is computationally expensive - hindering its practical adoption for industrial X-ray CT systems. 

\vspace{-0.25cm}
\subsection{Our solution}

We will disentangle the two problems -- beam-hardening artifacts, and sparse-view artifacts. 
Beam hardening is a projection domain phenomenon so we will correct it in that domain.
Sparse-view artifacts affect the detection of defects in the image domain, which is where we will correct this artifact.
We present a deep learning method to correct for both artifacts.

We propose a new linearization approach based on the use of a neural network (NN) to reduce BH.
We first train a NN to map between the projected value and estimated thickness to the parameters of Van de Casteel attenuation model \cite{van2002energy}.
During inference, the NN-estimated parameters of Van de Casteel model is then used to compute the linearization polynomial which is then used to correct the BH in the projection data.
The main advantage of our method is that once it is trained for a huge collection of (p, d) data points, it can be used to reduce BH for a range of materials. 
We demonstrate that it suppresses BH artifacts for numerous AM components made of different alloys without any manual tuning of the algorithm - enabling a fully automated workflow for X-ray CT of metal AM components to produce high-quality reconstructions. 
Furthermore, our beam hardening correction (BHC) method is robust against imperfect $p$ vs $d$ values due to an imprecise segmentation - a common occurrence for dense components with complex geometries.

We will leverage the superior quality of MBIR to reduce the sparse-view artifacts in the reconstruction image. MBIR can suppress these artifacts without compromising a lot on the image details.
We will design a NN that will be trained to use FDK images as input and furnish MBIR-quality images \cite{ziabari20182, rahman2021mbir}. 
To accomplish this we will train the network with training pairs of sparse-scan FDK image as input and dense-scan MBIR image as target. 
The network will learn a mapping from low-quality FDK to higher-quality MBIR images. 
This should result in reduction of noise and sparse-view artifacts, improvement of texture, and highlighting of the defects which is our primary goal.

\vspace{-0.5cm}


\vspace{-0.5cm}
\subsubsection{Inference}
Once the networks are trained, they can be used for reconstructing the X-ray CT data measured at the same resolution but with different setting and from different materials.
The input to the DL-MBIR network is a sparse-scan FDK reconstructed image that is beam hardening correction using BHCN.
The challenge is, as the materials become denser, the BH effect worsens, and also with the same measurement setting (energy, beam hardening filter, dwell time and averaging) the amount of light make it to the X-ray reduces (lower dosage), and therefore the result become noisier.
Therefore, very dense materials such as NiCo that are not seen during training, or Inconel that are seen during training but measured at a different setting, are considered out-of-distribution (OOD).
In the result section, we will demonstrate that our training strategy allows for high quality reconstruction of such out-of-distribution (OOD) data. 

